Resolving Molecular Contributions of Ion Channel Noise to Interspike Interval Variability through Stochastic Shielding

The contributions of independent noise sources to the variability of action potential timing has not previously been studied at the level of individual directed molecular transitions within a conductance-based model ion-state graph. The underlying connection provides an important example of how mathematics can be applied to study the effects of unobservable microscopic fluctuations to macroscopically observable quantities. We study a stochastic Langevin model and show how to resolve the individual contributions that each transition in the ion channel graph makes to the variance of the interspike interval (ISI). We extend the mean--return-time (MRT) phase reduction developed in (Cao et al. 2020, SIAM J. Appl. Math) to the second moment of the return time from an MRT isochron to itself. Because fixed-voltage spike-detection triggers do not correspond to MRT isochrons, the inter-phase interval (IPI) variance only approximates the ISI variance. We find the IPI variance and ISI variance agree to within a few percent when both can be computed. Moreover, we prove rigorously, and show numerically, that our expression for the IPI variance is accurate in the small noise (large system size) regime; our theory is exact in the limit of small noise. By selectively including the noise associated with only those few transitions responsible for most of the ISI variance, our analysis extends the stochastic shielding (SS) paradigm (Schmandt et al. 2012, Phys. Rev. Lett.) from the stationary voltage-clamp case to the current-clamp case. We show numerically that the SS approximation has a high degree of accuracy even for larger, physiologically relevant noise levels. We show that the ISI variance is not an unambiguously defined quantity, but depends on the choice of voltage level set as the spike-detection threshold, both in vitro and in silico.

==> 00README.XXX.tex <==
nohypertex
main.dvi keepcomments

==> base/ltfilehook-code.tex <==
% This will typeset documentation + code
%

\AtBeginDocument{\AlsoImplementation}
\input{ltfilehook.dtx}


==> base/ltfilehook-doc.tex <==
% This will typeset only documentation but not the code
%

\AtBeginDocument{\OnlyDescription
%                 \let\tableofcontents\relax
                 }
\input{ltfilehook.dtx}


==> base/lthooks-code.tex <==
% This will typeset documentation + code
%

\AtBeginDocument{\AlsoImplementation}
\input{lthooks.dtx}


==> base/lthooks-doc.tex <==
% This will typeset only documentation but not the code
%

\AtBeginDocument{\OnlyDescription
%                 \let\tableofcontents\relax
                 }
\input{lthooks.dtx}


==> base/ltshipout-code.tex <==
% This will typeset documentation + code
%

\AtBeginDocument{\AlsoImplementation}
\input{ltshipout.dtx}


==> base/ltshipout-doc.tex <==
% This will typeset only documentation but not the code
%

\AtBeginDocument{\OnlyDescription
%                 \let\tableofcontents\relax
                 }
\input{ltshipout.dtx}


==> base/ltxcheck.tex <==
% \iffalse meta-comment
%
% Copyright (C) 1993-2020
% The LaTeX3 Project and any individual authors listed elsewhere
% in this file.
%
% This file is part of the LaTeX base system.
% -------------------------------------------
%
% It may be distributed and/or modified under the
% conditions of the LaTeX Project Public License, either version 1.3c
% of this license or (at your option) any later version.
% The latest version of this license is in
%    https://www.latex-project.org/lppl.txt
% and version 1.3c or later is part of all distributions of LaTeX
% version 2008 or later.
%
% This file has the LPPL maintenance status "maintained".
%
% The list of all files belonging to the LaTeX base distribution is
% given in the file `manifest.txt'. See also `legal.txt' for additional
% information.
%
% The list of derived (unpacked) files belonging to the distribution
% and covered by LPPL is defined by the unpacking scripts (with
% extension .ins) which are part of the distribution.
%
% \fi
%
% \iffalse
%% File `ltxcheck.tex'.
%% Copyright (C) 1994-1997 LaTeX3 project, David Carlisle
%%
% LaTeX Test File.
% ================
%
% Processing this file with a newly installed LaTeX
% will test various aspects of the installation.
%
% To typeset the comments in this file, create a small
% file ltxcheck.drv that looks like the following (without the %)
%
%    \documentclass{ltxdoc}
%    \begin{document}
%    \DocInput{ltxcheck.tex}
%    \end{document}
%
% and process `latex ltxcheck.drv'.
%
\NeedsTeXFormat{LaTeX2e}[1997/06/01]
% \fi
%
% \StopEventually{}
% \CheckSum{643}
%
% \changes{v1.0c}{1994/03/15}
%         {Add \cmd{\NeedsTeXFormat}}
% \changes{v1.0t}{1996/09/25}
%         {Move ltxcheck to separate file}
% \changes{v1.0v}{1996/11/20}
%         {lowercase filenames /1044}
% \changes{v1.1d}{2004/02/11}
%         {Remove pict2e.sty}
%
\ProvidesFile{ltxcheck.tex}[2015/03/30 v1.1d LaTeX check file (DPC)]
%
% \GetFileInfo{ltxcheck.tex}
% \title{\textsf{ltxcheck}: The \LaTeX\ test program\thanks
%   {version~\fileversion, dated \filedate}}
% \author{David Carlisle}
% \date{\filedate}
% \MaintainedByLaTeXTeam{latex}
% \maketitle
%
% This file, |ltxcheck.tex| should be run after \LaTeX\ has been
% installed. It Checks some system dependent parts of \LaTeX\ are set up
% correctly for your system, and checks that the main input files and
% fonts that \LaTeX\ uses are present and can be found by \LaTeX.
%
%    \begin{macrocode}
\makeatletter
%    \end{macrocode}
%
%    \begin{macrocode}
\typeout{^^J%
LaTeX2e installation check file^^J%
===============================}
%    \end{macrocode}
%
%    \begin{macrocode}
\typeout{^^J%
 Before running this file through LaTeX2e you should have installed^^J%
 the Standard LaTeX files in their final `system' directories.^^J%
 This file should *not* be run in a directory that contains article.cls}
%    \end{macrocode}
%
% |\pause| just slows things down so that not too much appears on the
% screen at once, or scrolls off the top.
%    \begin{macrocode}
\def\pause{%
  \typeout{}%
  \message{** Hit return to continue: }%
  \read -1  to \xxx
  \typeout{}}
%    \end{macrocode}
%
%    \begin{macrocode}
\typeout{^^J%
  After certain tests, LaTeX will pause so that you can read the^^J%
  output without it scrolling off the screen.^^J%
  When you are ready just hit <return> and LaTeX will continue.^^J%
  When LaTeX pauses, you will see a prompt like the one below.^^J^^J%
  If a test fails, a message will be displayed followed by^^J%
  an error message starting `! BAD'.^^J%
  LaTeX will quit if you try to scroll past some error messages.}
\pause
%    \end{macrocode}
%
% Check that the system has defined |\@currdir| correctly
% by writing an |.aux| file and then trying to find it again.
%    \begin{macrocode}
\typeout{^^J%
  Checking the current directory syntax^^J%
  =====================================}
%    \end{macrocode}
%
%    \begin{macrocode}
\newif\iftest\testfalse
%    \end{macrocode}
%
%    \begin{macrocode}
\ifx\@currdir\@undefined
  \typeout{^^J%
  \noexpand\@currdir is undefined !!^^J%
  Something is seriously wrong with the LaTeX2e initialisation.^^J%
  Either you have corrupted files or this is a LaTeX bug.}
  \errmessage{BAD LaTeX2e system!!}
  \expandafter\@@end
\fi
%    \end{macrocode}
%
%    \begin{macrocode}
\ifx\@currdir\@empty
  \typeout{^^J%
  \noexpand\@currdir is defined to be empty.^^J%
  This means that LaTeX can not distinguish between a file^^J%
  aaaaa.tex^^J%
  that exists in the current directory, and  a file aaaaa.tex^^J%
  in another directory.^^J%
  It may be that this Operating System has no concept of `directory'^^J%
  in which case the setting is correct. If however it is possible to^^J%
  uniquely refer to a file then a suitable definition of
    \noexpand\@currdir^^J%
  should be added to texsys.cfg, and the format remade.}
  \pause
%    \end{macrocode}
%
%    \begin{macrocode}
\else
  \typeout{^^J%
\noexpand\@currdir is defined as
    \expandafter\strip@prefix\meaning\@currdir^^J%
  (Testing...)}
%    \end{macrocode}
%
%    \begin{macrocode}
\begingroup
\endlinechar=-1
\count@\time
\divide\count@ 60
\count2=-\count@
\multiply\count2 60
\advance\count2 \time
\edef\today{%
  \the\year/\two@digits{\the\month}/\two@digits{\the\day}:%
    \two@digits{\the\count@}:\two@digits{\the\count2}}
%    \end{macrocode}
%
%    \begin{macrocode}
  \immediate\openout15=ltxcheck.aux
  \immediate\write15{\today^^J}
  \immediate\closeout15 %
%    \end{macrocode}
%
%    \begin{macrocode}
  \openin\@inputcheck\@currdir ltxcheck.aux %
  \ifeof\@inputcheck
    \typeout{\@currdir ltxcheck.aux  not found}%
  \else
    \read\@inputcheck to \reserved@a
    \ifx\reserved@a\today
      \typeout{\@currdir ltxcheck.aux found}
      \testtrue
    \else
      \typeout{BAD: old file \reserved@a(should be \today)}%
      \testfalse
    \fi
  \fi
  \closein\@inputcheck
%    \end{macrocode}
%
%    \begin{macrocode}
  \iftest
    \endgroup
    \typeout{\noexpand \@currdir OK!}
  \else
  \endgroup
%    \end{macrocode}
%
%    \begin{macrocode}
  \typeout{^^J%
    The LaTeX2e installation has defined \noexpand\@currdir^^J%
    to be \expandafter\strip@prefix\meaning\@currdir.^^J%
    This appears to be incorrect.^^J%
    You should add a correct definition to texsys.cfg^^J%
    and rebuild the format.}
  \errmessage{BAD LaTeX2e system!!}
  \expandafter\expandafter\expandafter\@@end
  \fi
  \pause
%    \end{macrocode}
%
%    \begin{macrocode}
\fi
%    \end{macrocode}
%
% \changes{v1.0k}{1995/09/27}
%         {Check filename parser}
% Check the filename parser can at least cope with a simple
% name + extension, |article.cls|.
%    \begin{macrocode}
\typeout{^^J%
  Checking the filename parser^^J%
  ============================}
%    \end{macrocode}
%
%    \begin{macrocode}
\filename@parse{article.cls}
\def\reserved@a{article}
%    \end{macrocode}
%
%    \begin{macrocode}
\testtrue
\ifx\filename@base\reserved@a
  \ifx\filename@ext\@clsextension
  \else
    \testfalse
  \fi
\else
  \testfalse
\fi
\iftest
   \typeout{filename parser OK!}\pause
\else
  \typeout{^^J%
    The LaTeX2e installation has defined \noexpand\filename@parse.^^J%
    This appears to be incorrect.^^J%
    You should remove the incorrect definition from texsys.cfg^^J%
    and rebuild the format.}
  \errmessage{BAD LaTeX2e system!!}
  \expandafter\expandafter\expandafter\@@end
\fi
%
%    \end{macrocode}
%
% Check the input path by looking for |article.cls|. If |article.cls|
% is in the current directory it would be found anyway, so first check
% it is not there.
%    \begin{macrocode}
\typeout{^^J%
  Checking the input path^^J%
  =======================^^J}
%    \end{macrocode}
%
%    \begin{macrocode}
\begingroup
\let\input@path\@undefined
\ifx\@currdir\@empty\else
  \IfFileExists{\@currdir article.cls}
   {\typeout{%
      article.cls appears to be in current directory!^^J^^J%
      If this is the case, install article.cls into a^^J%
      `standard input directory'^^J%
      and copy ltxcheck.tex to another directory before^^J%
      processing with LaTeX.^^J%
      ^^J%
      If article.cls is not in the current directory,^^J%
      then you need to edit texsys.cfg.^^J%
      Read the comments in that file. If nothing else works, add:^^J%
      \string\let\string\@currdir\string\@empty^^J}%
    \errhelp{Move files, or edit texsys.cfg}
    \def\ArticleClassFoundInCurrentDirectory{%
      This file should not be run in a `standard input directory'}
    \errmessage{BAD: \ArticleClassFoundInCurrentDirectory}}
    {}
\fi
\endgroup
%    \end{macrocode}
%
%    \begin{macrocode}
\IfFileExists{article.cls}
  {\typeout{input path OK!}}
  {\typeout{^^J%
     LaTeX claims that article.cls is not on the system.^^J%
     Either LaTeX has been incorrectly installed, or the
     \noexpand\input@path^^J%
     is incorrect. A correct definition should be added to^^J%
     texsys.cfg, and the format remade.}
   \pause
   \typeout{^^J%
     Typical definitions of \noexpand\input@path include:^^J^^J%
     \string\let\string\input@path=\noexpand\@undefined
      (the default definition)^^J^^J%
     \string\def\string\input@path{\@percentchar^^J
       {/usr/lib/tex/inputs/} {/usr/local/lib/tex/inputs/} }^^J^^J%
     \string\def\string\input@path{\@percentchar^^J
       {c:/tex/inputs/} {a:/} }^^J^^J%
     \string\def\string\input@path{\@percentchar^^J
       {tex_inputs:} {SOMEDISK:[SOMEWHERE.TEX.INPUTS]} }^^J}%
   \pause
   \typeout{^^J%
     Note that \noexpand\input@path should be undefined
       unless your^^J%
     TeX installation does not make
       \noexpand\openin and \noexpand\input^^J%
     search the same directories.^^J%
     If \noexpand\input@path is defined, entries should be^^J%
     in the same syntax as \noexpand\@currdir^^J%
     ie full directory names that may be concatenated with the^^J%
     basename (note the final / and ] in the above examples).^^J%
     Some systems may need more complicated settings.^^J%
     See texsys.cfg for more examples.^^J%
    ! BAD \noexpand\input@path!!}
   \@@end}%
\pause
%    \end{macrocode}
%
% For versions prior to \TeX3 complain to the installer. (Although
% \LaTeX\ will work with these old \TeX\ versions).
% For versions between 3 and 3.14 check that \LaTeX\ is using the
% work-around for the |^^J| in |\message| bug.
%    \begin{macrocode}
\typeout{^^J%
  Checking the TeX version^^J%
  ========================}
%    \end{macrocode}
%
% \changes{v0.2j}{1994/02/25}
%         {\cs{noboundary} is \cs{relax} not undef in TeX2 (initialised
%         in 2e format)}
%    \begin{macrocode}
\dimen@\ifx\@TeXversion\@undefined4\else\@TeXversion\fi\p@%
\ifx\noboundary\relax
  \typeout{^^J%
    This is TeX 2. You will not be able to use all the new features^^J%
    of LaTeX2e with such an old TeX.^^J%
    The current version (1995/12/11) is TeX 3.14159.^^J%
    Consider upgrading your TeX.}
  \ifdim\dimen@<3\p@\else
     \errhelp{Check that texsys.cfg has not defined \@TeXversion}
     \def\OldTeX{%
       BAD: \noexpand\@TeXversion is incorrect: \meaning\@TeXversion}
     \errmessage{\OldTeX}
  \fi
\else
%    \end{macrocode}
%
% \changes{v1.0h}{1994/10/11}
%         {Check for TeX3.141}
%    \begin{macrocode}
    \ifdim\dimen@>3.14\p@
      \typeout{This appears to be a recent version of TeX!^^J%
       If the following `lines' all appear on the same line,^^J%
       separated by \string^\string^J %
       then there has been an incorrect installation.}
    \else
      \typeout{^^J%
       This appears to be a TeX between 3.0 and 3.14^^J%
       but the current version (1995/12/11) is TeX 3.14159^^J%
       consider upgrading your TeX.^^J%
       The following `lines' will appear on the same line,^^J%
       separated by \string^\string^J;^^J%
       the same problem may affect other messages from LaTeX.}
     \fi
%    \end{macrocode}
%
%    \begin{macrocode}
\message{line1^^Jline2^^Jline3}
\pause
%    \end{macrocode}
%
%    \begin{macrocode}
\fi
%    \end{macrocode}
%
%
% To check that the \LaTeX\ fonts have been installed, the well known
% trick of going into |\batchmode|, and testing for |\nullfont| is used.
% Not all fonts are tested, just a representative sample.
%    \begin{macrocode}
\typeout{^^J%
  Checking fonts^^J%
  =====================================}
%    \end{macrocode}
% \changes{v1.0h}{1994/10/11}
%         {Check for fonts}
%    \begin{macrocode}
\def\checkfont#1{%
  \batchmode
  \font\test=#1\relax
  \errorstopmode
  \ifx\test\nullfont
    \typeout{\@spaces! BAD: #1.tfm not found!}
    \@tempswatrue
  \else
    \typeout{\@spaces OK: #1.tfm found}
  \fi}
%    \end{macrocode}
%
%    \begin{macrocode}
\typeout{^^JChecking Standard TeX fonts...}
\@tempswafalse
\checkfont{cmr10}
\checkfont{cmr12}
\checkfont{cmmi10}
\if@tempswa
  \errhelp{Obtain a complete standard TeX font distribution.}
  \errmessage{BAD: Missing Standard Fonts}
\else
%    \end{macrocode}
% \changes{v1.0s}{1996/07/19}
%         {Check for bad cm fonts}
%    \begin{macrocode}
    \font\testcm=cmr10
    \testcm
    \setbox0\hbox{h{}o}
    \setbox2=\hbox{ho}
    \ifdim\wd0=\wd2
     \typeout{^^J%
OK: correct Computer Modern fonts installed.}%
    \else
     \typeout{^^J%
An unauthorised and incompatible release of the^^J%
Computer Modern fonts has been installed on your system.^^J%
The official fonts may be obtained from CTAN archives in:^^J%
ctan:fonts/cm^^J%
For further details see Donald Knuth's Home page:^^J%
http://www-cs-faculty.stanford.edu/\protect~knuth/cm.html}%
  \errhelp{Re-install Computer Modern fonts, and then rebuild LaTeX}
  \errmessage{BAD Standard fonts!!}
    \fi
%    \end{macrocode}
%
%    \begin{macrocode}
  \pause
\fi
%    \end{macrocode}
%
%    \begin{macrocode}
\typeout{^^JChecking LaTeX Picture Mode fonts...}
\@tempswafalse
\checkfont{lcircle10}
\checkfont{lcirclew10}
\if@tempswa
  \@tempswafalse
  \checkfont{circle10}
  \checkfont{circlew10}
  \if@tempswa
    \typeout{^^J! BAD: You do not have the picture mode fonts:^^J%
           lcircle10 and lcirclew10}
  \else
    \typeout{^^J! BAD:%
           You have the picture mode fonts with their old names:^^J%
           circle10 and circlew10 have been renamed to^^J%
           lcircle10 and lcirclew10}
  \fi
  \errhelp{Obtain a complete standard LaTeX font distribution.}
  \errmessage{BAD: Missing LaTeX Fonts}
\else
  \pause
\fi
%    \end{macrocode}
%
%    \begin{macrocode}
\typeout{^^JChecking Extra LaTeX Computer Modern fonts...}
\@tempswafalse
\checkfont{cmmib5}
\checkfont{cmmib7}
\checkfont{cmex7}
\if@tempswa
\typeout{! BAD:^^J%
 LaTeX2e uses a few `extra' Computer Modern fonts produced by^^J%
 The American Mathematical Society.^^J%
 If you install The AMSFONTS font collection, then these, and other,^^J%
 fonts will be available to LaTeX.^^J%
 Although installing AMSFONTS is recommended, LaTeX does not require^^J%
 The full collection; you may obtain a minimal set of extra LaTeX^^J%
 fonts from any CTAN archive, in: ctan:macros/latex/fonts/}
\errhelp{Obtain LaTeX fonts or  the AMSFONTS collection.}
\errmessage{BAD: Missing LaTeX Fonts}
\else
  \pause
\fi
%    \end{macrocode}
%
% \changes{v1.0k}{1995/09/27}
%         {Check for dc and tc fonts}
% \changes{v1.1a}{1997/01/14}
%         {Check for ec fonts}
% \changes{v1.1c}{1997/06/10}
%         {Modify messages now ec released}
%    \begin{macrocode}
\typeout{^^JChecking T1 encoded Computer Modern (dc & ec) fonts...}
%    \end{macrocode}
% \changes{v1.0m}{1995/10/31}
%         {Check the T1 fd files match the  dc release.}
% This command looks for the string |dcr17<| in the font tables for
% T1/cmr. If it is there, then the T1 fd files match the old dc fonts,
% for dc release 1.1 or earlier. If not then presumably new fd files
% are being used.
%    \begin{macrocode}
\def\dcrseventeen{%
  \begingroup
    \escapechar-1
    \xdef\reserved@a{%
      \noexpand\in@
        {\expandafter\string\csname dcr17\endcsname<}%
        {\expandafter\expandafter\expandafter
           \string\csname T1/cmr/m/n\endcsname<}}%
  \endgroup
  \reserved@a}
%    \end{macrocode}
% Similarly this command looks for the string |ecrm| in the font tables
% for T1/cmr. If it is there, then the T1 fd files match the ec fonts,
% for ec release 1.0 or later.
%    \begin{macrocode}
\def\ecrm{%
  \begingroup
    \escapechar-1
    \xdef\reserved@a{%
      \noexpand\in@
        {\expandafter\string\csname ecrm\endcsname}%
        {\expandafter\expandafter\expandafter
           \string\csname T1/cmr/m/n\endcsname}}%
  \endgroup
  \reserved@a}
%    \end{macrocode}
% \changes{v1.0o}{1995/11/14}
%    {dont produce a BAD message if just one set of dc fonts is missing}
% Remove the ``! BAD'' typeout while checking for dc fonts so
% as not to worry sites with just the new ones.
%    \begin{macrocode}
\def\checkfont#1{%
  \batchmode
  \font\test=#1\relax
  \errorstopmode
  \ifx\test\nullfont
    \typeout{\@spaces\@spaces #1.tfm not found}
    \@tempswatrue
  \else
    \typeout{\@spaces OK: #1.tfm found}
  \fi}
%    \end{macrocode}
%

%    \begin{macrocode}
\@tempswafalse
\checkfont{ecrm1000}
\if@tempswa
%    \end{macrocode}
% No ec fonts. Check the state of the dc fonts.
%
%    \begin{macrocode}
\typeout{No EC fonts found, checking DC fonts...}
\@tempswafalse
\checkfont{dcr10}
\if@tempswa
  \@tempswafalse
  \checkfont{tcr1000}
  \if@tempswa
%    \end{macrocode}
% No dc fonts at all.
%    \begin{macrocode}
    \typeout{^^J%
! BAD: No ec fonts found!!^^J%
LaTeX does not require the use of ec fonts^^J%
however they are strongly recommended.^^J%
The ec fonts are available in a more natural range of sizes^^J%
and allow better hyphenation and kerning than the^^J%
old fonts such as cmr10.^^J%
These ec fonts may be obtained from CTAN archives, in:^^J%
ctan:fonts/ec}
  \else
%    \end{macrocode}
% No old dc fonts, but new ones installed.
% First check whether the latest patch has been applied.
% \changes{v1.0p}{1995/12/11}
%         {Check for dc fonts 1.2 patch level 1 (Bernd Raichle) /2003}
% \changes{v1.0q}{1996/06/03}
%         {Check for dc fonts 1.3}
% \changes{v1.1b}{1997/01/24}
%         {extra closing brace removed from this branch}
%    \begin{macrocode}
    \font\testdc=dcr1000
    \testdc
    \setbox0\hbox{A{}y}
    \setbox2=\hbox{Ay}
    \ifdim\wd0>\wd2
     \typeout{^^J%
! BAD: dc fonts release 1.3 installed^^J%
The dc fonts are now replaced by the ec fonts^^J%
These ec fonts may be obtained from CTAN archives, in:^^J%
ctan:fonts/ec.}%
    \else
     \typeout{^^J%
! BAD dc fonts 1.2 or older installed.^^J%
The dc fonts are now replaced by the ec fonts^^J%
These ec fonts may be obtained from CTAN archives, in:^^J%
ctan:fonts/ec.}%
    \fi
    \dcrseventeen
    \ifin@
      \typeout{^^J%
The fd files for the obsolete release 1.1 of the^^J%
dc fonts have been loaded into the LaTeX format.^^J%
However, you appear to have at least release 1.2 of the dc fonts.^^J%
You should generate suitable fd files by running:^^J%
latex newdc.ins^^J%
and then rebuild the format by rerunning:^^J%
initex latex.ltx}
       \errmessage{BAD LaTeX2e system!!}
     \else
       \typeout{^^J%
         DC fonts OK!}
    \fi
  \fi
\else
  \@tempswafalse
  \checkfont{tcr1000}
  \if@tempswa
%    \end{macrocode}
% Old DC fonts, but no new ones.
%    \begin{macrocode}
    \typeout{^^J%
Old dc fonts found!!^^J%
Only the original dc fonts are on your system.^^J%
Later releases of the dc/ec fonts introduced^^J%
many improvements and are strongly recommended.^^J%
They may be obtained from CTAN archives, in:^^J%
ctan:fonts/ec.}
    \pause
    \dcrseventeen
    \ifin@\else
      \typeout{^^J%
The LaTeX2e installation has installed fd files for^^J%
release 1.2 (or later) of the dc fonts.^^J%
However, you appear to have only release 1.1 of these fonts.^^J%
You must now generate the correct fd files by running:^^J%
latex olddc.ins^^J%
and then rebuild the format by rerunning:^^J%
initex latex.ltx}
      \errmessage{BAD LaTeX2e system!!}
    \fi
  \else
%    \end{macrocode}
% Both old and new DC fonts.
%    \begin{macrocode}
    \font\testdc=dcr1000
    \testdc
    \setbox0\hbox{A{}y}
    \setbox2=\hbox{Ay}
    \ifdim\wd0>\wd2
     \typeout{^^J%
! BAD: dc fonts release 1.3 installed^^J%
The dc fonts are now replaced by the ec fonts^^J%
These ec fonts may be obtained from CTAN archives, in:^^J%
ctan:fonts/ec.}%
    \else
     \typeout{^^J%
! BAD dc fonts 1.2 or older installed.^^J%
The dc fonts are now replaced by the ec fonts^^J%
These ec fonts may be obtained from CTAN archives, in:^^J%
ctan:fonts/ec.}%
    \fi
%    \end{macrocode}
%
%    \begin{macrocode}
    \dcrseventeen
    \ifin@
      \typeout{^^J%
The fd files for the obsolete release 1.1 of the^^J%
dc fonts have been loaded into the LaTeX format.^^J%
However, you appear to have at least release 1.2 of the dcfonts.^^J%
You should use generate suitable fd files by running:^^J%
latex newdc.ins^^J%
and then rebuild the format by running:^^J%
initex latex.ltx^^J%
Otherwise LaTeX will always use the older fonts.}
       \errmessage{BAD LaTeX2e system!!}
    \else
      \ecrm
      \ifin@
        \typeout{^^J%
The fd files for the new EC fonts have been loaded into^^J%
the LaTeX format.^^J%
However, these fonts are not found by LaTeX.^^J%
You should either install the ec fonts, or generate suitable^^J%
fd files for the dc fonts by running: \space latex newdc.ins^^J%
and then rebuild the format by running: \space initex latex.ltx}
       \errmessage{BAD LaTeX2e system!!}
      \else
        \typeout{^^J%
DC fonts OK!^^J%
(Both old and new dc font releases are installed.)^^J%
Note that the dc fonts are expected to be replaced by ec^^J%
in January 1997.}
      \fi
    \fi
  \fi
\fi
%    \end{macrocode}
% Else EC fonts are found, so check whether LaTeX is going to use them.
%
%    \begin{macrocode}
\else
%    \end{macrocode}
%
%    \begin{macrocode}
  \ecrm
  \ifin@
   \typeout{EC fonts OK!}
  \else
    \typeout{%
EC fonts installed but LaTeX is still using dc fonts.^^J%
You may want to run ec.ins and remake the LaTeX format}
  \fi
%    \end{macrocode}
%
%    \begin{macrocode}
\fi
\pause
%    \end{macrocode}
%
%
%
% The following files will be unpacked by running iniTeX on
% |unpack.ins|.
%
%    \begin{macrocode}
\typeout{^^JChecking LaTeX input files...^^J}
%    \end{macrocode}
%
% If the specified file is not there, add it to the list.
%    \begin{macrocode}
\def\checkfile#1{%
  \IfFileExists{#1}{}{\edef\missingfile{\missingfile#1, }}}
%    \end{macrocode}
%
% Report any missing files in the last batch tested.
%    \begin{macrocode}
\def\filereport#1#2{%
\ifx\missingfile\@empty
 \typeout{^^J%
OK: The #1 files such as #2^^J%
are accessible to LaTeX.}
\pause
\expandafter\@gobbletwo
\else
  \typeout{^^J%
! BAD: The #1 files:^^J%
\missingfile^^J%
are not accessible to LaTeX.}
\errhelp{Check the installation!}
\let\missingfile\@empty
\fi
\errmessage{Missing LaTeX files}}
%    \end{macrocode}
%
% Kernel files:
%    \begin{macrocode}
\let\missingfile\@empty
%    \end{macrocode}
%
%    \begin{macrocode}
\checkfile{hyphen.ltx}
\checkfile{fontmath.ltx}
\checkfile{fonttext.ltx}
\checkfile{preload.ltx}
\checkfile{texsys.cfg}
\checkfile{latex.ltx}
%    \end{macrocode}
%
% Don't use |\filereport| here as the message is rather different
% as the |.ltx| files don't really need to be available to \LaTeX\
% once the format is made.
%    \begin{macrocode}
\ifx\missingfile\@empty
 \typeout{^^J%
OK: The files such as latex.ltx that are used to make^^J%
the format are  accessible to LaTeX.}
\else
  \typeout{^^J%
The files:^^J%
\missingfile^^J%
that are used to make the format are not accessible to LaTeX.^^J%
This is OK, but you will need those files if you need to remake the^^J%
the format later.}
\fi
\pause
\let\missingfile\@empty
%    \end{macrocode}
%
% Class files and class options:
%    \begin{macrocode}}
\checkfile{article.cls}
\checkfile{report.cls}
\checkfile{book.cls}
\checkfile{letter.cls}
\checkfile{ltxdoc.cls}
\checkfile{proc.cls}
\checkfile{slides.cls}
\checkfile{bk10.clo}
\checkfile{bk11.clo}
\checkfile{bk12.clo}
\checkfile{size10.clo}
\checkfile{size11.clo}
\checkfile{size12.clo}
\checkfile{fleqn.clo}
\checkfile{leqno.clo}
%    \end{macrocode}
%
%    \begin{macrocode}
\filereport{main class}{article.cls}
%    \end{macrocode}
%
% Package files:
%    \begin{macrocode}
\checkfile{alltt.sty}
\checkfile{doc.sty}
\checkfile{exscale.sty}
\checkfile{flafter.sty}
\checkfile{fontenc.sty}
\checkfile{graphpap.sty}
\checkfile{ifthen.sty}
\checkfile{inputenc.sty}
\checkfile{latexsym.sty}
\checkfile{makeidx.sty}
\checkfile{newlfont.sty}
\checkfile{oldlfont.sty}
\checkfile{shortvrb.sty}
\checkfile{showidx.sty}
\checkfile{slides.sty}
\checkfile{syntonly.sty}
\checkfile{tracefnt.sty}
%    \end{macrocode}
%
%
%    \begin{macrocode}
\filereport{main package}{ifthen.sty}
%    \end{macrocode}
%
% Font definition (.fd) files:
%    \begin{macrocode}}
\checkfile{omlcmm.fd}
\checkfile{omlcmr.fd}
\checkfile{omllcmm.fd}
\checkfile{omscmr.fd}
\checkfile{omscmsy.fd}
\checkfile{omslcmsy.fd}
\checkfile{omxcmex.fd}
\checkfile{omxlcmex.fd}
\checkfile{ot1cmdh.fd}
\checkfile{ot1cmfib.fd}
\checkfile{ot1cmfr.fd}
\checkfile{ot1cmr.fd}
\checkfile{ot1cmss.fd}
\checkfile{ot1cmtt.fd}
\checkfile{ot1cmvtt.fd}
\checkfile{ot1lcmss.fd}
\checkfile{ot1lcmtt.fd}
\checkfile{t1cmdh.fd}
\checkfile{t1cmfib.fd}
\checkfile{t1cmfr.fd}
\checkfile{t1cmr.fd}
\checkfile{t1cmss.fd}
\checkfile{t1cmtt.fd}
\checkfile{t1cmvtt.fd}
\checkfile{ts1cmr.fd}
\checkfile{ts1cmss.fd}
\checkfile{ts1cmtt.fd}
\checkfile{ts1cmvtt.fd}
\checkfile{ucmr.fd}
\checkfile{ucmss.fd}
\checkfile{ucmtt.fd}
\checkfile{ullasy.fd}
\checkfile{ulasy.fd}
%    \end{macrocode}
%
%
%    \begin{macrocode}
\filereport{font definition}{t1cmr.fd}
%    \end{macrocode}
%
% Font encoding files:
%    \begin{macrocode}
\checkfile{t1enc.def}
\checkfile{ot1enc.def}
\checkfile{omsenc.def}
\checkfile{omlenc.def}
%    \end{macrocode}
%
%
%    \begin{macrocode}
\filereport{font encoding}{t1enc.def}
%    \end{macrocode}
%
% Input encoding files:
%    \begin{macrocode}
\checkfile{ascii.def}
\checkfile{latin1.def}
\checkfile{latin2.def}
\checkfile{latin3.def}
\checkfile{latin5.def}
\checkfile{cp850.def}
\checkfile{cp852.def}
\checkfile{cp865.def}
\checkfile{cp437.def}
\checkfile{cp437de.def}
\checkfile{applemac.def}
\checkfile{next.def}
\checkfile{ansinew.def}
%    \end{macrocode}
%
%    \begin{macrocode}
\filereport{input encoding}{latin1.def}
%    \end{macrocode}
%
% Compatibility files:
%    \begin{macrocode}
\checkfile{article.sty}
\checkfile{book.sty}
\checkfile{letter.sty}
\checkfile{proc.sty}
\checkfile{report.sty}
\checkfile{fleqn.sty}
\checkfile{leqno.sty}
\checkfile{openbib.sty}
\checkfile{latex209.def}
%    \end{macrocode}
%
%
%    \begin{macrocode}
\filereport{compatibility mode}{article.sty}
%    \end{macrocode}
%
% Other files:
%    \begin{macrocode}
\checkfile{bezier.sty}
\checkfile{docstrip.tex}
\checkfile{slides.def}
\checkfile{sfonts.def}
\checkfile{t1enc.sty}
%    \end{macrocode}
%
%    \begin{macrocode}
\filereport{remaining}{sfonts.def}
%    \end{macrocode}
%
%    \begin{macrocode}
\@@end
%    \end{macrocode}
%
% \Finale
%

